Bogomolov property for modular Galois representations with nontrivial nebentypus

A field in which the (logarithmic) Weil height is bounded from below by a strictly positive constant is said to have the Bogomolov property (property (B)). Given a normalized eigenform $f\in S_k(\Gamma_0(N))$ Amoroso and Terracini proved (B) for the field "cut out" by the adelic representation associated to $f$ under some assumptions on $f$, generalizing the earlier work of Habegger on elliptic curves. In this paper we extend this result to the case of normalized eigenforms with nontrivial nebentypus character. We also introduce the notion of ADZ field, inspired by earlier work of Amoroso, David and Zannier, exhibiting a class of fields in which property (B) is preserved under (arbitrary) composition.

==> Diagramma.tex <==
\begin{tikzcd}
                                          & L(\varepsilon_p^{k-1}) \arrow[rd, no head] &                                                       \\
L \arrow[rd, no head] \arrow[ru, no head] &                                            & \mathbb{Q}_q(\varepsilon_p^{k-1}) \arrow[ld, no head] \\
                                          & \mathbb{Q}_q                               &                                                      
\end{tikzcd}
